Dynamic Planar Convex Hull

In this article, we determine the amortized computational complexity of the planar dynamic convex hull problem by querying. We present a data structure that maintains a set of n points in the plane under the insertion and deletion of points in amortized O(log n) time per operation. The space usage of the data structure is O(n). The data structure supports extreme point queries in a given direction, tangent queries through a given point, and queries for the neighboring points on the convex hull in O(log n) time. The extreme point queries can be used to decide whether or not a given line intersects the convex hull, and the tangent queries to determine whether a given point is inside the convex hull. We give a lower bound on the amortized asymptotic time complexity that matches the performance of this data structure.

==> intervaltree.tex <==
\begin{picture}(0,0)%
\includegraphics[scale=1]{./FIGintervaltree.pdf}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(5305,2195)(129,-2384)
\put(3076,-2311){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$q^*$}%
}}}}
\end{picture}%


==> pseudocode.tex <==
% pseudocode for topdown.tex, formated by alg2eformat.tex
\makeatletter
\catcode`\@=10

\def\myB{B}
@\defproc{replace}{Replace$_{\protect\myB}$}%
@@   {\arg{\wtype{point} r \ftype{\in B \subset \UH(A\cup B)}}\narg
@@     \arg{\wtype{list of points} L }}
@@   {\wret{list of locators}\fret{L'}=\hbox{}} 
@@   {\sit{there is a complete certificate with~$r$ --- for $A\cup B$} }
@@   {\res{there is a complete certificate with $L$ --- for $A\cup (B\cup L \setminus \{r\})$;\mynewline  $L'$ is replacement on  $\UH(A\cup B)$ } }
{ % #7
%\let\AlgFullCallWithOut\AlgFullCallWith
%\nl  \KwLet{$((X,Y\in A\cup B),(x,y\in B), O$ = \pc{remove($r$))} on $B$}\com{lOst}
\KwLet{$x,y\in B$ and $X,Y\in \UH(A\cup B)$ be the neighbors of~$r$}\;
\lnl{algrep:letLostEQ}\KwLet{ $e_x \in \overline{xr},e_y \in \overline{ry}$ be the lost equality on~$A$ or $\bot$ if $x$ or $y$ outside}\;
\AlgFullCallWithOut{rmBr}{(E_s,P)=}{r,X,Y}{algrep:rmBr}
\AlgFullCallWithOut{ApplySCn}{(\SC x,\SC y)=}{r,x,y,O,L}{algrep:applySC}
\lnl{algrep:ifReest}\If(\tcp*[f]{not everything above one shortcut}){$(\SC x,\SC y)\neq(\bot,\bot)$}{
  \AlgFullCallWithOut{reestablishBA}{(x',y')=}{\SC x,e_x,e_y,\SC y}{algrep:reestI}
  \AlgFullCallWithOut{reestablishAB}{(E,x'',y'')=}{\SC x,\SC y}{algrep:reestII}
  \nl\KwLet{\( (u_0,v_0) = (\mathrm{leftmost}\{x',x''\},\mathrm{rightmost}\{y',y''\})\)} \; 
  \AlgFullCallWithOut{CreateSC}{}{(u,v)}{algrep:createSC} 
}
\lnl{algrep:searchBr} \ForEach{$e \in (E \cap \hbox{slab of \(x\) and \(y\)} )\cup E_s$}{ 
  \AlgFullCallWithOut{FindBridge}{}{e,P}{algrep:findBr}
}
\lnl{algrep:return}\KwRet{locators of $\UH(A\cup B)$ between $X$ and $Y$ (by following bridges)}
}

@\defproc{FindBridge}{Find New Bridge}% old and new!!
@@   {\arg{\wtype{equality point} e \ftype{\subset \UH(B)\cap\UH(A)}}\narg
@@     \arg{\wtype{bypasses} P }}
@@   {\wret{}\fret{}} 
{ % #5
  \sit{$e$ is an equality point without bridge
    \mynewline 
    $P$ is a set of up to 4 bypasses}
}
{ % #6
  \res{A bridge is established above~$e$} % temporary
}
{ % #7
  % \com{uses and deletes wormholes}
  \KwLet $a\in \UV(A)$, $b\in \UV(B)$ be the outer neighbors of $e$
  % on $\DSinner$\;
  \com{$\overline{ab}$ above $e$}
  \Repeat{$\overline{ab}$ is bridge}
  {
    geometrically analyze $\overline{ab}$ as candidate bridge 
    \com{\cite{OvL81}}
    \If{$a$ is too far left}{
      % $a := a.\DSinner.right()$\; 
      change $a$ to the next input point to the right\;
      \com{jumping over cutting points and ray intersections}
      \If{$a == w.s$ for some $w\in P$\com{$a$ is endpoint of a bypass}}{ 
        $a:=w.t$ \com{follow the bypass}%\;
        % Remove bypass $w$ from $P$.\;
      }
    }
    $\ldots$ \com{symmetric for the other 3 possibilities:\\ \qquad $a$ too far right, $b$ too far left/right}\;
%    \qquad \com{$a$ too far right, $b$ too far left/right}\;
  }\;
  % Create temporary bridge right of $a$ and left of $b$ on \DSinner\;
  Establish in the data structure a bridge from $a$ to $b$ above~$e$\;
  % Create pointers from $a,b$ to $e$\;
  %\KwRet{$P$}\;
}
% sit{}: the point~$r$ on $\UV(A\cup B)\cap B$ is deleted (replaced)
% x,y,X,Y,
% %\res{$x,y$ neighbors of~$r$ on $B$, $X,Y$ neighbors on $\UH(A\cup B)$\mynewline
@\defproc{rmBr}{Remove}
@@    {\arg{\wtype{point} r \ftype{\in{B \cap \UH(A\cup B)}}} }
@@    {\wret{points, bypasses}\fret{(O,E_s,P)=\hbox{}}} 
@@    {\sit{$r$ is to be deleted from~$B$}}
@@    {\res{$O$ are all lost cutting points on $\overline{xry}$\mynewline
@@     $E_s$ equality points below bridges with endpoint~$r$, $P$ bypasses}}
{
  \KwLet{$x,y,X,Y, O$ as specified}\;
  Delete $r$ from the representation\;
  \KwSet{$E_s = P = \emptyset$}\tcp*{for bypasses}
  % (\tcp*[f]{see Figure~\ref{fig:protectors}})
  \lnl{alg:rmBr:foreach}
  \ForEach(\tcp*[f]{two per bridge}){endpoint~$c$ of affected bridge or equality~$e$}{ 
%    \KwLet{$e$ be the equality point below $\overline{Xr}$}\;
%    \KwLet{$b$} \com{outside, input point of~$B$ on $\UH(B)$}
    \eIf{$c\neq r$}{
      \KwLet{$t=c$}}{
      \KwLet{$t=x$ or $t=y$, the one under the bridge}
    }
    % (\tcp*[f]{$t$ })
    \If{$t$ is locally outside}{
      \KwLet{$s$ be the outside endpoint of the segment of~$e$ on the same set as~$t$}\;
      \KwSet{$P = P \cup \{ (s,t) \}$}
    }
    \If{$e$ is not affected}{
      \KwSet{$E_s = E_s \cup\{e\}$}\;
    }
  }
 \KwRet{$x,y,X,Y,O,E_s,P$}
}
@\defproc{ApplySCn}{Apply Shortcuts}
@@    {\arg{\wtype{point} x,y \ftype{\in{\UV(B)}}}
@@     \narg \arg{\wtype{lost pts} O \ftype{\in{\UH(B)}} }
@@     \narg \arg{\wtype{points} L \ftype{~}}}
@@    {\wret{points on $\SC B$}\fret{(\SC x,\SC y)=\hbox{}}}
@@    {  \sit{$L$ is to be placed between $x$ and $y$ on $B$ \mynewline
@@            $O$ lost cutting points (on $\overline{xry}$)}} 
@@    { \res{ the points ${\SC x},{\SC y} \in \SC B$ enclose all changes on $\SC B$\mynewline
@@        the data structure between ${\SC x}$ and ${\SC y}$ reflects the new~$\SC B$
@@        }
@@    }
{
  \com{The deleted point $r$ exists but is not part of the interface}
%  \KwLet{$x=$left$_B(r)$, $y=$right$_B(r)$}\;
  \KwSet{$({\SC x},{\SC y})=(x,y)$}\;
  \KwLet{$Z$ be the set of shortcuts intersecting $\overline{xry}$ with cutting points in $O$}\;
%  Delete $r$ and ray intersections on $\overline{xry}$ and $Z$\; % |Z|
%  \com{delete ray intersections, leave the selected point marked by a null-pointer $\bot$}
%  Delete cutting points on $\overline{xry}$\;
  % everything of $\SC B$ properly between ${x}$ and ${y}$
  \com{shortcuts of~$Z$ loose at least one cutting point}
  \KwLet{$F$ = ($x$ is marked as above shortcut \KwAnd{} $Z=\emptyset$)}\;
  \com{$F = $TRUE means $\overline{xry}$ is above some unknown shortcut}

  \ForEach{$b \in L$ from left to right}{
    Create base record and locator for $b$\;
    Connect $b$ into data structure of $B$ left of $y$\;
    \If{$F$ \KwOr{} $b$ is above some shortcut in $Z$}{
      Mark $b$ as above some shortcut\;
    }
  }
  \eIf{$F$}{
    \KwSet{$({\SC x},{\SC y})=(\bot,\bot)$}
  }{ 
    \ForEach{segment $(u,v)$ between $x$ and $y$ on~$B$}{
      \ForEach{shortcut~$\ell \in Z$}{
        \If{the line of $\ell$ crosses~$(u,v)$}{
          Create new cutting point of~$\ell$ in data structure\;
        }
      }
    }
    \If{$x$ is above a shortcut}{ 
      \KwLet{${\SC x}$ be the leftmost (new) cutting point of a shortcut in~$Z$}\;
      \com{see also Figure~\ref{fig:sc_appl}}
    }
    \If{$y$ is above a shortcut}{ 
      \KwLet{${\SC y}$ be the rightmost (new) cutting point of a shortcut in~$Z$}\;
    }
  }
  \ForEach{shortcut~$\ell \in Z$}{
    delete all ray intersections on $\ell$ \com{no need to remember them}
    \If{$\ell$ has no new cutting point}{
      delete (free) $\ell$ as shortcut
    } 
  }
 \KwRet{$({\SC x},{\SC y})$} \com{(staying) enclosing points of~$\SC B$ around $L$}
}

@\defproc{ApplySCold}{Old Apply Shortcuts}
@@    {\arg{\wtype{point} r \ftype{\in{\UV(B)}}}\narg
@@     \arg{\wtype{replacement points} L \ftype{~}}}
@@    {\wret{points on $\SC B$}\fret{(\SC x,\SC y)=\hbox{}}}
@@    {  \sit{$r$ is to be replaced by $L$ on $B$}} 
@@    { \res{    $L$ replaces $r$ in $B$\mynewline
@@        marked selected points in~$A$ with lost ray intersection (on $\overline{xr}$, $\overline{ry}$ or shortcut)\mynewline
@@        the points ${\SC x},{\SC y} \in \SC B$ enclose all changes on $\SC B$\mynewline
@@        the data structure between ${\SC x}$ and ${\SC y}$ reflects the new~$\SC B$
@@        }
@@    }
{
  \KwSet{$x=r.leftNgbB()$, $y=r.rightNgbB()$}\com{typeset!}\;
  \eIf{$x,r,y$ are above a shortcut (and marked) and there is no cutting point on $\overline{xry}$}{ 
    \KwSet{$({\SC x},{\SC y}) = (\bot,\bot)$} \com{certificate still valid}\;
    \KwSet{$Z=\emptyset$}\com{rather: line way below}\;
  }{ 
    \KwLet{$({\SC x},{\SC y}) = (x,y)$}\;
    \If{$y$ is above a shortcut}{ 
      \KwLet{$v$ be the rightmost cutting point on $\overline{xry}$}\;
      \KwLet{${\SC y} = \ v.leftNgbB$}\com{not on $\overline{xry}$, inside, remains}\;
      \com{ref Figure! right endpoint of SC?}
    }
    \If{$x$ is above a shortcut}{ 
      $\ldots$, symmetric for~${\SC x}$\;
    }
    \KwLet{$Z$ be the set of shortcuts with cutting points on  $\overline{xry}$}\;
  }
  Delete $r$ and everything of $\SC B$ properly between ${\SC x}$ and ${\SC y}$\;
  \hfill\com{cutting points of shortcuts in $Z$, ray intersections}\;
  \ForEach{$b \in L$}{
    Create base record for $b$\com{locator?}\;
    Connect $b$ into doubly linked list of $B$\;
    \If{$b$ above some shortcut in $Z$ or $({\SC x},{\SC y})=(\bot,\bot)$}{mark~$b$ as a above shortcut}
  }
  \ForEach{$\overline{uv} \in \{x\} \cup L \cup \{y\}$\com{if Z not empty}}{
    \If{$\overline{uv}$ cuts a shortcut $l \in Z$}{
      Create cutting point for $l$ including pointers
    }
  }
  Free shortcuts in $Z$ that became obsolete\;
 \KwRet{${\SC x},{\SC y}$} \com{(staying) enclosing points of~$B$ around $\SC L$}
}

@\defproc{CreateSC}{Create Shortcuts} 
@@    {\arg{\wtype{locally outside points} u_0,v_0}}
@@    {}
@@    { \sit{$u_0,v_0$ enclose all new ray intersections and equalities}} 
@@    { \res{the set of shortcuts $H_A,H_B$ are (again) aggressive}}
{
  \ForEach{pair $(u,v)$ of neighboring ray intersections or equality points on (scan) the locally outer \textbf{shortcut} hull between $u_0$ and $v_0$ }{
    \ForEach{input point $c$ on the \textbf{shortcut} hull $\UH(\SC A)\cup\UH(\SC B)\setminus (A\cap B)$ between $u$ and $v$}{\KwSet{$c$ as hidden by a shortcut}}
    \lForEach{shortcut $s$ \textbf{properly} between $u,v$}{delete $s$}
    \KwLet{$x,y$ be the extreme input points between $u,v$}\tcp*{see Fig.~\ref{fig:createSC}}
    \KwSet{$x$ and $y$ as not hidden by a shortcut}\;%\tcp*{do nothing if non-existing}
    \If{$x$ and $y$ are not neighbors}{
      Create shortcut $\overline{xy}$ and mark both points as cutting points.
    }
  }
}

\def\mathBA{$^B_A$}
@\defproc{reestablishBA}{reestablish\mathBA}
@@    {\arg{\wtype{points} \SC x,e_x,e_y,\SC y \in \SC B}}
@@    {\wret{points}\fret{(x',y')=\hbox{}}}
{ \sit{$\SC B$ represents $\SC L$ between $\SC x$ and $\SC y$\mynewline
    If $\SC x$ is inside, $e_x$ is leftmost lost equality (on A), $\SC y$ symmetric\mynewline
    $A$ has lost equality / missing ray intersections between $\SC x,\SC y\!\!\!\!$}%(in data structure)}
}{ \res{new certificate for all streaks $B$ above $A$ between $\SC x,\SC y\!\!\!\!$\mynewline
    $x',y'\in \SC B$ enclose all new ray intersections and equality points.}
}
{
  \eIf{$\SC x$ is outside}{
    \lnl{alg:reestablishBA:extend}
    \KwLet{$p\in A$ and $\RrayP{p} \in \SC B$ be the first to the left $A$--$B$-connection:\\
      \quad selected point~$p$ -- ray intersection $\RrayP{p}$ OR equality point $p=\RrayP{p}=e$}\;
  }(\tcp*[f]{\hspace{.7cm}$\SC x$ inside, $e_x \neq \bot$\hspace{5.2cm}}){
    \lnl{alg:reestablishBA:lostEq}
    \KwLet{$p=e_x\in A$ and $\RrayP{p}\in \SC B$ the point straight below~$p$}\;
    \com{scan on $\SC B$ from $\SC x$ to the right, locally inside}
  }
  \KwLet{$q\in A,\LrayP{q} \in B$ be defined symmetrically based on $\SC y, e_y$}\;
  \lnl{alg:reestablishBA:scanT}
  \KwLet{$T$ be the points of~$\SC B$ between $\RrayP{p}$ and $\LrayP{q}$}
  \tcp*{one scan on $\SC B$}
  \lnl{alg:reestablishBA:split}
  \KwLet{$p_0=p,p_1,\ldots,p_k=q$ the constantly many (previously) selected points and lost equality points of~$A$ including $e_x,e_y$ between $p$ and $q$}
  \tcp*{mini (jumping splitters) scan on $\SC A$}
  \For{$i=0\ldots k-2$}{
    \KwSet{$(T_i,T) =$ \pc{split}$(T,p_{i+1}$)}\tcp*{at vertical line through $p_{i+1}$}
    \KwSet{$\LrayP{p_{i+1}}=\RrayP{p_{i+1}}$ on the segment of $\SC B$ at this split}
    \tcp*{above or below}
%    \AlgFullCallWith{refineBA}{}{p_i,p_{i+1},\RrayP{p_i},\LrayP{p_{i+1}},T_i}{sbwlew}
    \pcwoX{refineBA}{p_i,p_{i+1},\RrayP{p_i},\LrayP{p_{i+1}},T_i}
  }
  \pcwoX{refineBA}{p_{k-1},p_{k},\RrayP{p_{k-1}},\LrayP{p_{k}},T}
  \KwRet{$\RrayP{p},\LrayP{q}$}
}

\def\mathAB{$^A_B$}
@\defproc{reestablishAB}{reestablish\mathAB}
@@    {\arg{\wtype{points} \SC x,\SC y}}
@@    {\wret{equalities, points}\fret{(E,x'',y'')=\hbox{}}}
@@    { \sit{all new/changed equalities $E$ are represented in DS
@@        \mynewline all streaks $B$ above $A$ have valid certificates
@@        \mynewline $\SC x,\SC y$ enclose replacing $\SC L$ as part of $\SC B$ (using old shortcuts)}} 
@@    { \res{All streaks $A$ above $B$ have new certificate;\mynewline
@@         all new/changed equality points are returned \mynewline points $x'',y''\in \SC A$ (outside) enclose new certificates.} } 
{
%  \com{TODO: change to $x',y'$?}
  \lnl{alg:reestablishAB:scan}
  \KwLet{$E$ be the equality points on $\SC B$ between $\SC x$ and $\SC y$}
  \tcp*{one scan}
  \lnl{alg:reestablishAB:newCS}
  \ForEach{pair $e_l,e_r \in E$ delimiting one streak $S$ with $A$ above $B$}{
    \KwLet{$T$ be a split-array of $\SC A$ between $e_l$ and $e_r$}%\;
    \tcp*{mostly new outside}
    Place points of $B$ between $e_l$ and $e_r$ into a splitter\;
    \hbox{\pcwoX{refineAB}{e_l,e_r, e_l,e_r,T}, adjust $x'',y''$ 
    \tcp*{new or previously trivial}}
  }
  \lnl{alg:reestablishAB:adjustRay}
  \If(\tcp*[f]{adjust ray}){$x$ is selected (and inside)}{%\com{means $x$ is inside}
    \KwLet{$p$ be the left next selected or equality point ($e=p=\RrayP{p}$) of $x$}\;
    %\com{\# does exist?}
    adjust $\Lray{x}$ and ray intersection $\LrayI{x}$ with $\SC A$
    \tcp*{few points on $\SC A$,}
    \KwLet{$T$ be a split array of $\SC A$ between $\RrayP{p}$ and $\LrayI{x}$}%\;
    \tcp*{i.e. constant}
    \hbox{\pcwoX{refineAB}{p,x,\RrayP{p},\LrayI{x},T}%
      , \KwSet{$x''= \RrayP{p}$}}
  }
  \lIf(\tcp*[f]{symmetric to the previous}){$y$ is selected}{$\ldots$}
  \lnl{alg:reestablishAB:adjustEq}
  \If(\tcp*[f]{$x$ is inside}){leftmost $e$ of $E$ is right end of $S$ with $A$ above $B$}{
    \KwLet{$p\in B$ next selected left of~$e$}%
    \tcp*{$p=x$ or via splitter of $x$}
    \KwLet{split array $T$ for $\SC A$ between $\RrayI{p}$ and $e$}
    \tcp*{mostly new outside}
    \hbox{\pcwoX{refineAB}{p,e,\RrayI{p},e,T}%{alg:reestAB:callExt}
      , adjust $x'',y''$}
  }
  \lnl{alg:reestablishAB:join}
  \lIf{rightmost $e$ of $E$ is left end of streak $S$ with $A$ above $B$}{$\ldots$}
  \If{$E=\emptyset$ and $\SC x$ (and $\SC y$) is inside $A$ }{
    \KwLet{$M_p$ splitter with  endpoint~$x$}%
    \tcp*{$M_p=\{p=x\}$ if $x$ is selected}
    \KwLet{$M_q$ be the splitter with left endpoint~$y$}
    \tcp*{$M_p$ and $M_q$ are open}
    \KwSet{$M=$ \pc{Join}$(M_p,L,M_q)$} as part of the data structure\;
    \KwLet{split array $T$ of $\SC A$ between $\RrayI{p}$ and $\LrayI{q}$}
    \tcp*{mostly new outside}
%    \AlgFullCallWith{refineAB}{}{x,y,\RrayI{x},\LrayI{y},T}{alg:reestAB:callJoin}
    \hbox{\pcwoX{refineAB}{p,q,\RrayI{p},\LrayI{q},T}, adjust $x'',y''$}
  }
 \KwRet{$E,x'',y''$}
}

@\defproc{refineBA}{refine\mathBA}
@@    {\arg{\wtype{construction site} p,q \in \UH(A), \RrayP{p},\LrayP{q} \in \SC B, T \subset \SC B}} 
@@    {}
@@    { \sit{The construction site with
@@             selected or equality points $p,q$,\mynewline
@@             alignment intersection \(\RrayP{p},\LrayP{q}\),
@@             % splitter between $p,q$ 
@@             and split array $T$ }}
@@    {\res{All parts of a streak of polarity $A$ above $B$ between $p$ and $q$ have a valid certificate}}
{             
  \If{$\RrayP{p}$ is vertically above $p$}{
    \lnl{alg:refineBA:shootRay}
    Establish ray intersection $\RrayI{p}$ (shoot right ray), see Section~\ref{sec:shootRay}\;
    \hbox{\pcwo{refineBA}($p,q,\RrayI{p},\LrayP{q},T$)}
    \KwRet{}
  }
  \lIf{$\LrayP{q}$ is above $q$}{$\ldots$ \hbox{\pcwo{refineBA}($p,q,\RrayP{p},\LrayI{q},T$)}\,\,\KwRet \tcp*[f]{symmetric}}
  \eIf(\tcp*[f]{$p$ or $q$ selected}){$p$ or $q$ is inverted and $M$ is closed}{
    \lnl{alg:refineBA:open}
    Define colors $C$ of $M$, inv. empty, other previous, see Sect.~\ref{sec:openInverted}\;
    % \KwGoto{Line~\ref{alg:refineBA:searchSplit}}
  }
  {
    \If(\tcp*[f]{$M$ is open}){$\RrayP{p}$ is below $p$ (inverted)}{
      \lnl{alg:refineBA:scanEq}
      Scan for equality~$e$, shortening~$M$ and $T$, see~Section~\ref{sec:scanEq}\;
      \lIf(\tcp*[f]{ow no $B$ above~$A$}){$e$ left of~$q$}{\hbox to 2cm{\pcwo{refineBA}($e,q,e,\LrayP{q},T$)}}
      \KwRet{}
    }
    \lIf{$\LrayP{q}$ is below $q$}{$\ldots$ \hbox{\pcwo{refineBA}($p,e,\RrayP{p},e,T$)}\,\,\KwRet \tcp*[f]{symmetric}}
    \lnl{alg:refineBA:finishBoundary}
    \lIf(\tcp*[f]{See Sect.~\ref{sec:finishBoundary}}){$p,q$ form a valid boundary certificate}{\KwRet\!\!}
    \lnl{alg:refineBA:searchSplit}
    \tcp{Now:\hspace{1.25ex}\hbox{$p,q$ selected or equality, rays established, see~Sect.~\ref{sec:searchSplitBA}}}
    Def. colors ${\mathcal C}$ of $M$ by shadows: red by $\RrayI{p}$, blue by $\LrayI{q}$, or eq~$=\emptyset$\;
  }
  $(M_1,o,M_2) =$ \pc{split}($M,{\mathcal C}$), in data structure\; % (will succeed if inv.)\;
  \If(\tcp*[f]{tangent certificate not valid, always if eq. pt. or inv.}){$o \neq \bot$}{
    \lnl{alg:refineBA:vertical}
    $(T_1,T_2) =$  \pc{split}($T,o$), defining $\LrayP{o}=\RrayP{o}$\tcp*[f]{possibly inside}\;
    {\hbox{\pcwo{refineBA}($p,o,\RrayI{p},\LrayP{o},T_1$) }} %{{\qquad\tcp*{$p$ is in its own shadow, so {$p\neq o$}}}}
    {\hbox{\pcwo{refineBA}($o,q,\RrayP{o},\LrayI{q},T_2$) }} %{{\qquad\tcp*{$q$ is in its own shadow, so {$o\neq q$}}}}
  }
  \KwRet{}
}

\def\mathAB{$^A_B$}

@\defproc{refineAB}{refine\mathAB}
@@    {\arg{\wtype{construction site} p,q\in \UH(B),\RrayP{p},\LrayP{q}\in \SC A,T \subset \SC A}}
@@    {}
@@    { \sit{The construction site of polarity $A$ above $B$ with
@@             selected or equality points $p,q$, %\mynewline
@@             alignment intersection \(\RrayP{p},\LrayP{q}\),
@@             %the splitter between $p,q$ and 
@@             split array $T$}}
@@    {\res{The data structure describes a certificate of\mynewline polarity $B$ above $A$ between $p$ and $q$}}
{             
  \KwLet{$M$ be the splitter between $p$ and $q$}\com{$M$ can be open or closed}
  % \;\com{if $M$ is closed, $p,q$ are selected points with established rays}
  \lnl{alg:refineAB:shootRay}
  \If{$\RrayP{p}$ is vertically above $p$}{
    Establish ray intersection $\RrayI{p}$ (shoot right ray), see Section~\ref{sec:shootRay}\;
    \hbox{\pcwo{refineAB}($p,q,\RrayI{p},\LrayP{q},T$)}
    \KwRet{}
  }
  % (//{symmetric for $q,\LrayP{q}$})
  \lIf{$\LrayP{q}$ is vertically above $q$}{$\ldots$ \hbox{\pcwo{refineAB}($\ldots$)}\,\,\KwRet \tcp*[f]{symmetric}}
  %\If(\tcp*[f]{symmetric to $p,\RrayP{p}$}){$\LrayP{q}$ is (vertically) above $q$}{$\ldots$}
  \lnl{alg:refineAB:finishBoundary}
  \lIf(\tcp*[f]{See Section~\ref{sec:finishBoundary}}){$p,q$ form a valid boundary certificate}{\KwRet}
  \tcp{Now: \hbox{$p,q$ selected or equality, rays established, see~Section~\ref{sec:searchSplit}}}
  \lnl{alg:refineAB:searchSplit}
  Def. colors ${\mathcal C}$ of $M$ by shadows: red by $\RrayI{p}$, blue by $\LrayI{q}$, equality empty\;
  $(M_1,o,M_2) =$ \pc{split}($M,{\mathcal C}$) in data structure\;
  \If(\tcp*[f]{tangent certificate not valid, always if eq. pt.}){$o \neq \bot$}{
    $(T_1,T_2) =$  \pc{split}($T,o$), defining $\LrayP{o}=\RrayP{o}$\;
    {\hbox{\pcwo{refineAB}($p,o,\RrayI{p},\LrayP{o},T_1$)\quad\tcp*{selected $p$ is in its own shadow, so {$p\neq o$}}}}
    {\hbox{\pcwo{refineAB}($o,q,\RrayP{o},\LrayI{q},T_2$)\quad\tcp*{selected $q$ is in its own shadow, so {$o\neq q$}}}}
  }
  \KwRet{}
}

@\defproc ABCDEFG

\makeatother


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: topdown.tex
%%% TeX-master: "topdown"
%%% outline-regexp: "[{ ]*\\\\\\(defproc{\\|arg{\\|wret{\\)"
%%% outline-regexp: "[{ ]*\\(\\\\\\(defproc{\\|arg{\\|wret{\\)\\|{\\)"
%%% outline-regexp: "[ ]+"
%%% outline-regexp: "[@]+"
%%% outline-level: outline-level
%%% End:

